Route-Time Conflict Maps for Cooperative End-to-End Autonomous Driving

Existing cooperative end-to-end driving works at Class A (status-sharing) of the SAE J3216 classes of cooperative driving automation (CDA): vehicles exchange what they perceive, not what they intend, so each plans alone when to go, which limits cooperation and leads to deadlock when both vehicles yield or to collisions when both go. We present When2Go, a cooperative end-to-end driving system that learns when to go by sharing intent under CDA Class B or higher. Each vehicle broadcasts its LiDAR detections with forecast motion as instance tokens, together with its plan and intended trajectory. The receiver draws the fused detections, forecasts and partner plans into a route-time conflict map, the occupancy along its route over the planning horizon, on which a planner scores candidate speed profiles. Where two intended trajectories conflict, an order gate, a precedence network distilled from a right-of-way rule, decides who goes first; both vehicles evaluate it on the same messages and so reach the same order. When2Go imitates the rule-based expert of V2Xverse, which sees the simulator's ground truth; stops that When2Go cannot observe within its 2 s planning horizon are relabelled, so that it does not learn to wait without an observable cause. For our runs only, the benchmarks' PID controller steers by When2Go's waypoints instead of the route, and its forced push of long-waiting vehicles is off. With one model, When2Go sets the state of the art on three closed-loop CARLA benchmarks: 97.8 and 90.7 driving score on InterDrive without and with traffic (best published 90.1 and 78.9), 70.0 on the public V2Xverse protocol (best of sixteen rerun methods 59.1) and 88.2 on MDrive (best rerun 85.1), with 95.0% of its vehicles collision-free (87.7%).

==> figs/pipe/pipe_scene3d_leader.tex <==
\def\scEgoU{0.4858}\def\scEgoV{0.7763}
\def\scPlanU{0.5453}\def\scPlanV{0.7074}
\def\scCarZeroU{0.3349}\def\scCarZeroV{1.1229}
\def\scCarTwoU{0.6096}\def\scCarTwoV{0.2812}
\def\scCarThreeU{0.6585}\def\scCarThreeV{0.1962}
\def\scGhostU{0.5639}\def\scGhostV{0.5311}
\def\scZoneU{0.5301}\def\scZoneV{0.5420}
\def\scPpathU{0.5447}\def\scPpathV{0.4692}
\def\scMsgCarTwoU{0.6565}\def\scMsgCarTwoV{0.6701}
\def\scMsgCarThreeU{0.6732}\def\scMsgCarThreeV{0.6412}

